An Entropy-Stable/Double-Flux scheme for the multi-component compressible Navier-Stokes equations

We present a novel combination of numerical techniques to improve the efficiency, accuracy, and robustness of multi-component compressible flow simulations. At the core of our approach is an Entropy-Stable formulation that preserves kinetic energy and integrates a Double-Flux scheme tailored for multi-component flows with variable specific heat ratios. This formulation yields low-dissipation, oscillation-free solutions and enhances stability compared to standard fully conservative methods. To further improve robustness, we introduce a new hybrid dissipation strategy that blends the Entropy-Stable/Double-Flux approach with conventional dissipation mechanisms. We provide a rigorous proof that the resulting numerical flux satisfies a semi-discrete entropy inequality, ensuring consistency with the second law of thermodynamics. For time integration, we employ an explicit Runge-Kutta scheme in combination with adaptive mesh refinement to capture local flow features dynamically. The method is implemented within an existing compressible Navier-Stokes solver based on OpenFOAM. Benchmark cases, including multi-dimensional interface and shock-interface interactions, demonstrate the effectiveness of the proposed framework. The results confirm its favorable stability and robustness, validating the approach as a promising advancement for high-fidelity simulations of supersonic flows.

==> sections/algorithms/algorithm1.tex <==
\begin{algorithm}[H]
\textbf{Input}:
	$v_{i_1\ldots i_d} \in \mathbb{R}^{n_1 \times \cdots \times n_d}$,
	$J_{l_1\ldots l_d} \in \mathbb{R}^{\tilde{n}_1 \times \cdots \times \tilde{n}_d}$,
	$B_{i_k j_k} \in \mathbb{R}^{\tilde{n}_k \times \tilde{n}_k}$ and
	$M_{l_k j_k} \in \mathbb{R}^{\tilde{n}_k \times n_k}$\\
\textbf{Output}: $v^\prime_{i_1\dots i_d} \in \mathbb{R}^{n_1\times \cdots \times n_d}$
\begin{algorithmic}[1]
	\State $V_{j_1\ldots j_d} 		\leftarrow L^{-1}_{ i_1  j_1}\cdots L^{-1}_{ i_d  j_d} v_{ i_1\ldots i_d }$	\Comment{Preconditioning from right}
	\State $X_{k_1\ldots k_d} 	\leftarrow M_{k_1 j_1}\cdots M_{k_d j_d} V_{j_1\ldots j_d}$
	\State $Y_{l_1\ldots l_d} 	\leftarrow \invinterpmat{ k_1}{l_1 }\cdots \invinterpmat{ k_d}{l_d } X_{k_1\ldots k_d}$	\Comment{Use $\mat L \mat U$-factorization of $ \mat{B}_k, \; k=1,...,d$}
	\State $Y^\prime_{l_1\ldots l_d} \leftarrow J_{l_1\ldots l_d} \odot Y_{l_1\ldots l_d}$
	\State $Z^\prime_{k_1\ldots k_d} \leftarrow {\hat \Gamma}_{ k_1\ldots k_d l_1\ldots l_d} Y^\prime_{l_1\ldots l_d}$		\Comment{Evaluate in parallel without forming $\mat{\Gamma}$}
	\State $Z_{k_1\ldots k_d} \leftarrow J_{k_1\ldots k_d} \odot Z^\prime_{k_1\ldots k_d}$
	\State $Y_{j_1\ldots j_d} \leftarrow \invinterpmat{ j_1 }{  k_1 }\cdots \invinterpmat{ j_d }{ k_d } Z_{k_1\ldots k_d}$ 	\Comment{Use $\mat L \mat U$-factorization of $ \mat{B}_k, \; k=1,...,d$}
	\State $V_{l_1\ldots l_d} \leftarrow M_{j_1 l_1}\cdots M_{j_d l_d} Y_{j_1\ldots j_d}$
	\State $v_{i_1\ldots i_d}^\prime \leftarrow L^{-1}_{i_1 l_1}\cdots L^{-1}_{i_d l_d} V_{l_1\ldots l_d}$
  \Comment{Preconditioning from left}
\caption{Matrix-free evaluation of the matrix-vector product $\mat{v}^\prime \mapsto \mat{\tilde{A}}^\prime \mat{v}^\prime $}\label{alg:mf_eval}
\end{algorithmic}
\end{algorithm}


==> settings/mycommands.tex <==
%% Abkürzungen
\newcommand{\NYS}{Nystr{\"o}m\xspace}
\newcommand{\BEZ}{B{\'e}zier\xspace}
\newcommand{\Lame}{Lam{\'e}\xspace} % Lame


%% Format of vectors, matrices and spaces
\newcommand{\myMat}[1]{\mathbf{#1}}
\newcommand{\mySpace}[1]{\mathcal{#1}}
\newcommand{\myVec}[1]{\mathbf{#1}}
\newcommand{\myVecGreek}[1]{\boldsymbol{#1}}
\newcommand{\myNorm}[1]{\lVert #1 \rVert}
\newcommand{\myCardinality}[1]{\# #1}

%% general indices
\newcommand\indexA{i} 		% first normal index
\newcommand\totalA{I} 		% total number of elements of index A
\newcommand\indexB{j} 		% second normal index
\newcommand\totalB{J} 		% total number of elements of index B
\newcommand\indexC{k} 		% third normal index
\newcommand\totalC{K} 		% total number of elements of index C
\newcommand\indexD{m} 		% forth normal index
\newcommand\totalD{M} 		% total number of elements of index D
\newcommand\indexE{n} 		% forth normal index
\newcommand\totalE{N} 		% total number of elements of index E
\newcommand\indexF{t} 		% forth normal index
\newcommand\totalF{T} 		% total number of elements of index F
\newcommand\indexG{l} 		% forth normal index
% \newcommand\indexG{\ell} 		% forth normal index
\newcommand\totalG{L} 		% total number of elements of index G

%% specifiv indices
% \newcommand\indexGauss{g}
% \newcommand\totalGauss{n}
\newcommand\indexGauss{q}
\newcommand\totalGauss{Q}
\newcommand\indexSpan{s}	% index of span of B-spline segment
\newcommand\indexSpanTrimmed{t}	% index of trimmed span of B-spline segment
\newcommand{\indexLevel}{\ell}	% index for the refinement level
\newcommand{\totalLevel}{L}	% index for the refinement level


%% multi index
\newcommand\mIndexI{\myVec{i}}
\newcommand\mIndexJ{\myVec{j}}
\newcommand\mIndexP{\myVec{p}}
% \newcommand\mIndexA{\myVec{i}} 	% multi index
% \newcommand\mTotalA{\myMat{I}} 	% multi index
% \newcommand\mIndexB{\myVec{j}} 	% multi index
% \newcommand\mIndexP{\myVec{p}}	% multi index


%% NURBS 
\newcommand{\Bspline}{B} 		% symbol for B-spline
\newcommand{\BsplineSeg}{\mathcal{B}} 	% symbol for B-spline segment
% \newcommand{\BsplineSeg}{S}} 	% symbol for B-spline segment
\newcommand{\NURBS}{R} 			% symbol for NURBS
\newcommand{\KV}{\varXi} 		% knot vector
\newcommand{\KVRefined}{\hat{\varXi}} 	% knot vector refined
\newcommand{\KVC}{\varLambda} 		% knot vector of the Cauchy data - nystroem
\newcommand\uu{\xi} 			% Local NURBS coordinates
\newcommand\uuRefined{\hat{\uu}} 	% inserted knots
\newcommand\vv{\uu} 			% Local NURBS coordinates
\newcommand\UVsurf{\pt{\uu}} 	% Local NURBS coordinates
\newcommand\uusurf{\uu_1} 		% Local NURBS coordinates
\newcommand\vvsurf{\vv_2} 		% Local NURBS coordinates
\newcommand\uuc{a} 			% Local NURBS coordinates for artificial knot vector  of the Cauchy data
\newcommand\multi{m} 			% Multiplicity of a knot
% \newcommand{\w}{w} 			% symbol for the NURBS weights
% \newcommand{\W}{\w(\uu)} 		% symbol for NURBS weighting function
\newcommand{\knotinsertion}{d_k}

\newcommand\refElXi{r}                  % coordinates of the reference element

%% point types
\newcommand{\CP}{\pt{c}}		% control points
\newcommand{\CPRefined}{\hat{\CP}} 	% refined control point
\newcommand{\CPara}{c}			% control parameter
\newcommand{\CPH}{\CP^h} 		% homogeneous control point
\newcommand{\CPHRefined}{\hat{\CP}^h} 	% homogeneous control point
\newcommand{\CPCoons}{\CP^{\uu}}	% control points for local Coons patch
\newcommand\collocationPoint{\pt{x}^c}	% collocation point
\newcommand\collocationPointNys{\collocationPoint}	% collocation point
\newcommand{\GP}{\pt{y}} 		% quadrature point

%% abscissa
\newcommand\abscissa{\bar{\uu}}			% abscissa
\newcommand\abscissaAnyDim{\bar{\pt{\uu}}}	% abscissa general dimension
\newcommand\greville{\abscissa}		% Greville abscissa
% \newcommand\greville{\abscissa^g}		% Greville abscissa
\newcommand\grevilleAnyDim{\bar{\pt{\uu}}^g}	% Greville abscissa general dimension
\newcommand\demko{\abscissa^d}		% Demko abscissa
\newcommand\uuExtended{\abscissa^e}	% Local NURBS coordinates and Greville
\newcommand\abscissaShift{\alpha}	% offset for discontinuous basis functions (2-ring)
% \newcommand{\discontinuousShift}{\hat{\alpha}} % shift of abscissa (not 2-ring approach)
\newcommand\collocP{\bar{\uu}^c}	% symbol for collocation points

%% spaces
\newcommand{\BsplineSpace}{\mathbb{S}} % symbol for B-spline space
\newcommand{\ApproxSpace}{\mathbb{S}_h}% symbol for B-spline space
\newcommand{\SolutionSpace}{\mathbb{S}} % symbol for B-spline space

%% degrees and order
\newcommand\pu{p}			% NURBS degree on u
\newcommand\polyorder{\tilde{\pu}}	% polynomial order on u
\newcommand\pv{p_{v}}			% NURBS degree on v
\newcommand\puc{p_{q}}			% nystroem quadratur order on u
\newcommand\puCauchy{\pu_c}		% degree of Cauchy data basis
\newcommand\puGeo{\pu_g}		% degree of Geometry basis
\newcommand\pusurf{\pu_1} 		% Local NURBS degree
\newcommand\pvsurf{\pu_2} 		% Local NURBS degree

%% patch types
% \newcommand{\curve}{\pt{x}\operate{\uu}}
\newcommand{\curve}{\pt{C}}
% \newcommand{\curve}{{\tau}}
% \newcommand{\curveRefined}{\hat{\pt{x}}\operate{\uu}}
% \newcommand{\curveRefined}{\hat{\pt{x}}}
\newcommand{\curveRefined}{\hat{\curve}}
% \newcommand{\curveBez}{\pt{x}_{b}}%%\operate{\xi_1}}
\newcommand{\curveBez}{{\tau}_{b}}%%\operate{\xi_1}}
% \newcommand{\curveBezOpposite}{\pt{x}_{e}}%%\operate{\xi_1}}
\newcommand{\curveBezOpposite}{{\tau}_{e}}%%\operate{\xi_1}}

%% element types
\newcommand\gradingSubEl{\ell} 		% # of sub-elements introduced by grading
% \newcommand\be{\omega} 			% boundary element (NURBS)
\newcommand\be{\gamma} 			% boundary element (NURBS)
% \newcommand{\IGAel}{e_\uu} 		% integration element
\newcommand\ieKs{\tau} 		% non-zero knot span
\newcommand\ieLocal{\tilde{\ieKs}} 		% local integration element for EXTENDED B-splines
% \newcommand\ieg{\tilde{\ieKs}} 		% Element for Gauss integration
% \newcommand\iegLocal{\grave{\ieKs}} 	% Local element for Gauss integration
\newcommand\ieReference{\grave{\ieKs}} % reference element [-1,1]

% \newcommand\ieKs{\tau^{\emptyset}} % non-zero knot span
% \newcommand\ieAr{\tau^{\boxtimes}} % integration region with aspect ratio 1
% \newcommand\ie{\tau^{\boxplus}} % sub-element of hierarchically refined%

% \newcommand\ieKs{\tau^{\square}} % non-zero knot span
% \newcommand\ieAr{\tau^{\boxplus}} % integration region with aspect ratio 1
% \newcommand\ie{\tau^{\boxdot}} % sub-element of hierarchically refined

% \newcommand\ieAr{\hat{\tau}^{\boxplus}} % integration region with aspect ratio 1
% \newcommand\ie{\hat{\tau}^{\boxdot}} % sub-element of hierarchically refined
%\newcommand\ie{\hat{\tau}^{\boxdot}} % sub-element of hierarchically refined




%% Extended B-splines
\newcommand{\exBspline}{B^e} 		% symbol for extended B-spline
\newcommand{\degSet}{\mathbb{J}} 	% symbol for the set of degenerated B-splines
% \newcommand{\degSet}{\eta} 	% symbol for the set of degenerated B-splines
\newcommand{\innerSet}{\mathbb{I}} 	% symbol for the set of degenerated B-splines
\newcommand{\exteriorSet}{\mathbb{K}} 	% symbol for the set of degenerated B-splines
\newcommand{\NSet}{\mathbb{T}} 	  	% symbol for the set of knot Menge for Nbasis
\newcommand{\eweight}{e} 	  	% symbol for the extrapolation weight
\newcommand{\Nbasis}{\psi} 	  	% symbol for newton's basis
\newcommand{\taylorpoint}{\tilde{\uu}} % extension point for taylor expansion
% \newcommand{\poly}{\gamma} 		% factor of a polynomial: \poly_1 * x + \poly_2 
\newcommand{\poly}{{\alpha}} 		% factor of a polynomial: \poly_1 * x + \poly_2 
\newcommand{\lambdapoint}{\mu} 	% extension point for deBoorFix functional
% \newcommand{\lambdapoint}{\upsilon} 	% extension point for deBoorFix functional
\newcommand{\trim}{t}
\newcommand{\variableKnot}{\hat{\uu}}

%% Extended THB-splines
\newcommand{\refinementCriterion}{c_e}  % symbol for the refinement criterion which determines the extrapolation length
\newcommand{\extrapolationLength}{d_e}
\newcommand{\knotSpanSize}{h_{\uu}}
\newcommand{\refinementLevel}{\ell}
\newcommand{\abscissaFineScale}{\abscissa^{(\refinementLevel+1)}}
\newcommand{\subCoef}{\alpha}


%% independent field approximation 
\newcommand{\GeoBasis}{\theta} 		% basis funtion related to the geometry field
% \newcommand{\PrimaryBasis}{\varphi} 	% basis funtion related to the primary field
% \newcommand{\DualBasis}{\psi} 		% basis funtion related to the dual field
\newcommand{\PrimaryBasis}{\Bspline^{\primary}} 	% basis funtion related to the primary field
\newcommand{\DualBasis}{\Bspline^{\dual}} 		% basis funtion related to the dual field
\newcommand{\sub}{s} 		%% sub-indices for sub-parametric formulations
\newcommand{\iso}{i} 		%% sub-indices iso-parametric formulations



%% Nyström
\newcommand{\LCNadmissibility}{\eta} 	% symbol for local correction admissibility factor
\newcommand{\LCNarea}{\Omega_{\collocationPointNys}}



%% local refinement
\newcommand{\locRefInfo}{\grave{\pt{\uu}}} % point for local refinement
\newcommand{\transMatrix}{\mathbf{T}}
\newcommand{\nodeMatrix}{\mathbf{N}}
\newcommand{\nodeMatrixLocal}{\nodeMatrix^{\ell}}
\newcommand\Lieg{l} 
\newcommand\LiegLocal{l}



%% analysis stuff
% \newcommand{\hoelder}{\gamma} 		% Hölder constant
\newcommand{\hoelder}{\upsilon} 		% Hölder constant
\newcommand{\DOF}{n} 			% symbol for degrees of freedom
\newcommand\cdim{d}			% Cartesian dimension
\newcommand\KVdim{\delta}			% Cartesian dimension
\newcommand{\domain}{\Omega}
% \newcommand{\patchdomain}{\Omega^{\textnormal{v}}}
\newcommand{\patchdomain}{\mathcal{A}^{\textnormal{v}}}
% \newcommand{\patchdomain}{\Gamma_{\textnormal{v}}}
\newcommand{\boundary}{\Gamma}
\newcommand{\boundaryNonSmooth}{\boundary^0}
\newcommand{\Ltwo}{L_{2}}
\newcommand{\GramDet}{G}
\newcommand\primary{u} 			% primary variable - displacements in elasticity
\newcommand\primaryApprox {\primary_h} % primary variable - displacements in elasticity
\newcommand\dual{t} 			% dual variable - tractions in elasticity
\newcommand\utens{\primary} 		% displacement tensor field
\newcommand\ttens{\dual} 		% surface traction tensor
\newcommand\conductivity {k} 		% conductivity
\newcommand\uvek{\myVec{u}} 		% displacement vector field
\newcommand\tvek{\myVec{t}} 		% surface traction
\newcommand\uvekc{\tilde{\uvek}} 	% displacement vector at control points
\newcommand\tvekc{\tilde{\tvek}} %	 traction at control points


\newcommand{\LshapeCoord}{\zeta} 		% symbol for degrees of freedom

%% Real numbers
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}

%% mappings
\newcommand{\perspectiveMap}{\op{P}}

%% math operators
\DeclareMathOperator{\sgn}{sgn}
% \DeclareMathOperator{\dx}{d}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\troot}{root}
\DeclareMathOperator{\dist}{\mathrm{dist}}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\diag}{diag}

%% Integral Operator
\newcommand\op[1]{\mathcal{#1}}
\newcommand\operate[1]{(#1)}
\newcommand\dx[1]{\;\text{d}#1}

%% H-matrices
\newcommand{\rk}{\mathcal{R}_k} % Low Rank Matrices
\newcommand{\h}{\mathcal{H}} % Hierarchical
\newcommand{\hmatrix}{\mbox{$\h$-matrix}\xspace}
\newcommand{\hmatrices}{\mbox{$\h$-matrices}\xspace}
% \newcommand{\rkm}{\rk-} % Low Rank Matrices
\newcommand{\orderof}[1]{\mathcal{O}\left(#1\right)} % Landau Symbol
% \newcommand{\storage}[1]{\mathsf{St}\left(#1\right)} % Storage
% \newcommand{\operations}[2]{\mathsf{Op}_{\mathit{#1}}\left(#2\right)}
% Operations
\newcommand{\order}{\mathcal{O}} % Landau Symbol only
\newcommand{\storage}{\mathsf{St}} % Storage 
\newcommand{\operations}{\mathsf{Op}} % Operations



%% URLs
\providecommand\url[1]{\emph{#1}}
% \newcommand\url[1]{\emph{#1}}


%% Signum-function
%\newcommand\sig[1]{\operatorname{sign} \left( #1 \right)} 



%% Integrals with any sign in the middle
%% (see Latex Symbels AMS p105.
\newcommand\Xint[1]{\mathchoice {\XXint\displaystyle\textstyle{#1}}%
  {\XXint\textstyle\scriptstyle{#1}}%
  {\XXint\scriptstyle\scriptscriptstyle{#1}}%
  {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
  \!\int}
\newcommand\XXint[3]{{\setbox0=\hbox{$#1{#2#3}{\int}$}
    \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
%\newcommand\ddashint{\Xint{=}} %% dashed integral
\newcommand\dashint{\Xint{-}} %% double sashed integral


%\newcommand\cpvint{-\!\!\!\!\!\!\!\!\!\int}
%\newcommand\cpvint{\dashint}
\newcommand\cpvint{\Xint{c}}
%\newcommand\cpvint{\strokedint}

\newcommand\mymin[1]{\min\{#1\}}
\newcommand\mymax[1]{\max\{#1\}}
\newcommand\fromto[2]{\{ #1, \dots, #2 \}}
\newcommand\mal{\cdot}




%% Differential Operators
\renewcommand{\div}{\nabla \cdot}
\newcommand{\grad}{\nabla}
\newcommand{\curl}{\nabla \times}
\newcommand{\Laplace}{\Delta}
\newcommand{\dTr}{\op{T}} %% conormal derivative

\newcommand\dgamma[1]{\dx\mathrm{s}_{\pt{#1}}}
\newcommand\domega[1]{\dx{\pt{#1}}}


%\newcommand{\Tr}{\mathrm{Tr}} %% boundary trace
% \newcommand{\dTr}{\op{T}} %% conormal derivative

%% Vector and matrix notation
% \newcommand\vek[1]{\mathbf{#1}}
% \newcommand\veks[1]{\boldsymbol{#1}}
% \newcommand\mat[1]{\mathbf{#1}}
\newcommand\tens[2]{\mathsf{#1}}
% 
\newcommand{\trans}{\intercal} % transposed matrix/vector
\newcommand{\inv}{{-1}} % inverted matrix

%% Abbreviations



\newcommand\ct{T} % cluster tree
\newcommand\bct{T_{I\times J}} % block cluster tree

%\newcommand\fund[3]{\tens{#1}{#2}{][
\newcommand\fund[1]{\tens{#1}{2}}
% \newcommand\fund[2]{\tens{#1}{2}{\ofpt{#2}}}
% \newcommand\fund[3]{\tens{#1}{2}\left(\pt{#2},\pt{#3})}

\newcommand\dirac{\delta}
\newcommand\kronecker{\delta}





%% Text in math
\newcommand\beistrich{,\,}
%\newcommand\with{\quad\text{with}\,}
\newcommand\und{\,\text{and}\,}
\newcommand\oder{\,\text{or}\,}
\newcommand\with{\,\text{with}\,}
\newcommand\for{\,\text{for}\,}
\newcommand\where{\,\text{where}\,}

%% Points
% \newcommand\pt[1]{\veks{#1}}
% \newcommand\pt[1]{\myVec{#1}}
\newcommand\pt[1]{\boldsymbol{#1}}
\newcommand\ofpt[1]{(\pt{#1})}
% \newcommand\ofpt[1]{(\pt{#1})}
\newcommand\sourcept{\tilde{\pt{x}}}
\newcommand\fieldpt{\hat{\pt{x}}}
\newcommand\boundarypt{\pt{y}}


%% Symbols
\newcommand\eps{\varepsilon}
\newcommand\err{\epsilon}
\newcommand\residual{\err}
\newcommand\mychi{\mathcal{X}}

%% Todo-list
\newcommand\done{\checkmark}

%% Figures
\newcommand{\myfig}[4]{
  % file=#1, size=#2, caption=#3, label=#4
  \begin{figure}[ht]%[htb!]
    \centering
    \includegraphics[width=#2]{#1}
    \caption{#3}
    \label{fig:#4}
  \end{figure}
}


\ifdefined\tikzSubmission
%% TikZ Figure with relative scaling to full linewidth (tikzscale-package)
\newcommand{\tikzfig}[5]{
  % file=#1, size=#2, caption=#3, label=#4, figno=#5
%   \begin{figure}[ht]%[htb!]
    \centering
    \includegraphics{#5}
    \caption{#3}
    \label{fig:#4}
%   \end{figure}
}
\else
%% TikZ Figure with absolute scaling
\newcommand{\tikzfig}[5]{
  % file=#1, size=#2, caption=#3, label=#4, figno=#5
%   \begin{figure}[htb!]

    \def\tkzscale{#2}
    \def\dirtikz{tikz} % define tikz directory
    \def\dirdata{data} % define data directory
    \centering
    \tikzsetnextfilename{#5}
    \input{#1}
    \caption{#3}
    \label{#4}
%   \end{figure}
}
\fi

%% add Tikz Subfigure
\ifdefined\tikzSubmission
\newcommand{\tikzsubfig}[5]{
    % file=#1, size=#2, subcaption=#3, label=#4, figno=#5
    \centering
    \includegraphics{#5}%
    \subcaption{#3}
    \label{#4}
}
\else
\newcommand{\tikzsubfig}[5]{
  % file=#1, size=#2, subcaption=#3, label=#4, figno=#5

    \def\tkzscale{#2}
    \def\dirtikz{tikz} % define tikz directory
    \def\dirdata{data} % define data directory
    \centering
    \tikzsetnextfilename{#5}
    \input{#1}
    \subcaption{#3}
    \label{#4}
}
\fi


%% Tables
\newenvironment{mytable}[4]%
{
  % #1=position #2=caption #3=label #4=table layout
  \begin{table}[#1]%[htb!]
    % \caption{#1}
    % \label{tab:#2}
    \def\mycap{#2}
    \def\mylabel{#3}
    \centering
    \begin{tabular}{#4}
      \toprule
%       #4 \\ 
%       \midrule
%       \hline%\noalign{\smallskip}
}
{
  %\noalign{\smallskip}
%   \hline
  \bottomrule
  \end{tabular}
  \caption{\mycap}
  \label{\mylabel}
  \end{table}
}
\newcommand{\mytableheader}[1]{
  % #1=header without line breaks (i.e. ' 1.col & 2.col & 3.col ' )
       #1 \\ \midrule
}

\newenvironment{mytableposition}[4]%
{
  % #1=caption #2=label #3=table layout #4=position
  \begin{table}[#4]%[htb!]
    % \caption{#1}
    % \label{tab:#2}
    \def\mycap{#1}
    \def\mylabel{tab:#2}
    \centering
    \begin{tabular}{#3}
      \toprule
%       #4 \\ 
%       \midrule
%       \hline%\noalign{\smallskip}
}
{
  %\noalign{\smallskip}
%   \hline
  \bottomrule
  \end{tabular}
  \caption{\mycap}
  \label{\mylabel}
  \end{table}
}
% \newcommand{\mytableheader}[1]{
%   % #1=header without line breaks (i.e. ' 1.col & 2.col & 3.col ' )
%        #1 \\ \midrule
% }






%% Algorithms
% % Algorithm comment style
% \newcommand{\store}{=} 	% symbol for storing with in algorithm
% \newcommand{\myinsert}{\leftarrow} 	% symbol for insertions with in algorithm
% % \renewcommand{\algorithmiccomment}[1]{\hspace{1cm} // #1} 
% \renewcommand{\algorithmiccomment}[1]{\hspace{1cm}$\vartriangleright$ #1} 
% % Algorithm environment
% \newenvironment{myalgorithm}[2]%
% {
%   % #1=caption #2=label
%   \begin{algorithm}
%     \caption{#1}
%     \label{#2}
%     \begin{algorithmic}[1]
% }   
% {
% \end{algorithmic}
% \end{algorithm}
% }

%% Todo-List
% \ifdefined\tikzSubmission
% \newcommand\todos[2]{ %
% }
% \else
% \newcommand\todos[2]{ %
% {
%   \ifdefined\tikzExtOn
%   \tikzset{external/export=false}
%   \fi
%   \todo[inline,size=\scriptsize,caption={List:
%     #1}]{ \begin{minipage}{\linewidth} #2 \end{minipage} } 
% }
% }
% \fi

% % Personalized comments
% \ifdefined\tikzSubmission
% \newcommand{\mycomment}[2][-]{ }%
% \else
% \newcommand{\mycomment}[2][-]{%
%   % initials of the author (optional) + note in the margin
%   {%
%     {
%     \ifdefined\tikzExtOn
%     \tikzset{external/export=false}
%     \fi
%     \setstretch{0.7}% spacing
%     \todo[color={green!33},size=\scriptsize]{
%       \textbf{[\uppercase{#1}]} #2}}%
%   }
% }%
% \fi


%% References to insert
% \ifdefined\tikzSubmission
% \newcommand{\todoref}[2][reference]{}
% \else
% \newcommand{\todoref}[2][reference]{%
%   {
%   \ifdefined\tikzExtOn
%   \tikzset{external/export=false}
%   \fi
%   \todo[color=blue!50,size=\scriptsize]{\emph{#2} #1}[{\color{blue!50}{\textsl{#2}}}]
% }
% }%
% \fi

\newcommand{\mychangeEq}[1]{\color{red}\textbf{#1}\color{black}}
% \newcommand{\mychangeEq}[1]{#1}
\newcommand{\mychange}[1]{\color{red}\textbf{#1}\color{black}\xspace}
% \newcommand{\mychange}[1]{\color{red}{#1}\color{black}\xspace}
% \newcommand{\mychange}[1]{\protect\hl{#1}}

\ifdefined\TodoNotes
    %%% Marked revisions and annotations
    \newcommand{\mycomment}[2][-] % works for okular too
    {
    %   \pdfcomment[color=yellow,voffset=3pt,opacity=0.75,author=#1]{#2}
%       \ignorespaces
        {%
            \ifdefined\tikzExtOn
            \tikzset{external/export=false}
            \fi
%             \setstretch{0.1}% spacing
            \todo[color={green!33}]{ \textbf{[\uppercase{#1}]} #2}
            \pdfcomment[color=yellow,opacity=0.0,author=#1]{}%% invisible comment to show comment in annotations list
        }%
    }	
    % \sethlcolor{green} % set highlight color to green
    \newcommand{\myhighlight}[2][-] % works for okular too
    {
    \pdfcomment[color=yellow,voffset=-5pt,hoffset=3pt,opacity=0.0,author=#1]{}%% invisible comment to show highlight in annotations list
    \hl{#2}%
    }	
    \setstcolor{red} % set strike out color to red
    \newcommand{\mydelete}[2][-] % works for okular too
    {
    \pdfcomment[color=yellow,voffset=-5pt,hoffset=3pt,opacity=0.0,author=#1]{}%% invisible comment to show highlight in annotations list
    \st{#2}%
    }
\else
    \newcommand{\mycomment}[2][-]{}
    \newcommand{\myhighlight}[2][-]{}
    \newcommand{\mydelete}[2][-]{}
\fi

\ifdefined\tikzSubmission
\newcommand\revdel[2]{}
\newcommand\revadd[2]{}
\newcommand\revmod[2]{}
\newcommand\revcomment[1]{} % for cases where pdfmarkupcomment does not work (i.e. figures)
\else
\newcommand\revdel[2]{ %
{
  \pdfmarkupcomment[markup=StrikeOut,color=red,author=Marussig and Zechner]{#1}{#2}
}
}
\newcommand\revadd[2]{ %
{
  \pdfmarkupcomment[markup=Underline,color=green,author=Marussig and Zechner]{#1}{#2}
}
}
\newcommand\revmod[2]{ %
{
  \pdfmarkupcomment[markup=Highlight,color=yellow,author=Marussig and Zechner]{#1}{#2}
}
}
\newcommand\revcomment[1]{ %
{
  \pdfcomment[color=yellow,author=Marussig and Zechner,voffset=8pt,opacity=0.8]{#1}
}
}
\fi




%% Theorems and remarks
% \theoremstyle{remark}
% \newtheorem*{remark}{Remark}
\newtheoremstyle{myremark}% ⟨name⟩ 
{3pt}% Space above
{3pt}% Space below
{}% Body font
{}% Indent amount
{\itshape}% Theorem head font
{:}% Punctuation after theorem head
{.5em}% Space after theorem head
{}% Theorem head spec (can be left empty, meaning ‘normal’)
\theoremstyle{myremark}
\newtheorem*{remark}{Remark}

%% References
\newcommand{\myEqref}[1]{Equation~(\ref{#1})}
\newcommand{\myeqref}[1]{equation~(\ref{#1})}	
\newcommand{\myfigref}[1]{Figure~\ref{#1}}
\newcommand{\myFigref}[1]{Figure~\ref{#1}}
\newcommand{\myRef}[1]{(\ref{#1})}
\newcommand{\mytabref}[1]{Table~\ref{#1}}
\newcommand{\myTabref}[1]{Table~\ref{#1}}
\newcommand{\mySecref}[1]{Section~\ref{#1}}
\newcommand{\mysecref}[1]{Section~\ref{#1}}
\newcommand{\myalgref}[1]{Algorithm~\ref{#1}}
% \newcommand{\myEqref}[1]{Equation~(\ref{#1})}
% \newcommand{\appref}[1]{\ref{#1}}
% \newcommand{\myappref}[1]{Appendix~\ref{#1}}
\newcommand{\myappref}[1]{\ref{#1}}
% \newcommand{\myAppref}[1]{Appendix~\ref{#1}}
\newcommand{\myAppref}[1]{\ref{#1}}
\newcommand{\mychapref}[1]{Chapter~\ref{#1}}
\newcommand{\myChapref}[1]{Chapter~\ref{#1}}

%% Comp. Mech format
% \newcommand{\figref}[1]{Fig.~\ref{#1}}
% \newcommand{\secref}[1]{Sect.~\ref{#1}}
% \newcommand{\chapref}[1]{Chap.~\ref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}
% \renewcommand{\algref}[1]{Algorithm~\ref{#1}}

%% Standard format
% \newcommand{\figref}[1]{Figure~\ref{#1}}
% \newcommand{\Figref}[1]{Figure~\ref{#1}}
% \newcommand{\secref}[1]{section~\ref{#1}}
% \newcommand{\Secref}[1]{Section~\ref{#1}}
% \newcommand{\chapref}[1]{chapter~\ref{#1}}
% \newcommand{\Chapref}[1]{Chapter~\ref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}
% \newcommand{\Tabref}[1]{Table~\ref{#1}}
% \providecommand{\algref}[1]{Algorithm~\ref{#1}}
% \renewcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\Algref}[1]{Algorithm~\ref{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Other commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Input from standard input path
\newcommand{\myinput}[1]{%
  \input{\CommonPath/#1}
}



%% footnotes
\newcounter{footnoteNumber} % initialization of counter with 0
\newcommand{\myfootnote}[1]
{% -> needed to avoid space between word and footnotemark
  \addtocounter{footnoteNumber}{1}%
  \footnotemark[\value{footnoteNumber}]%
  \footnotetext[\value{footnoteNumber}]{#1}%
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 


==> settings/myheadings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % myheadings.tex
% %
% % 	requires:		\usepackage{scrpage2}
% % 				\usepackage{setspace}
% %

%%% Headings
%\pagestyle{headings}
\automark[chapter]{section}
\pagestyle{scrheadings}
% \rehead{\chaptermark}
\chead{}
\rohead[]{\pagemark}
%\rohead{\pagemark}
%\lohead{\rightmark}
\lohead{\rightmark}
\rehead{\leftmark}
% \lehead{}
\lehead{\pagemark}
\lefoot{}
\cefoot[]{}
\cofoot[]{}
% \rofoot[\pagemark]{\pagemark}
\rofoot[]{}
\setheadsepline{1pt}

%%% Vertical offset of chapters (standard is 1.8)
\renewcommand*{\chapterheadstartvskip}{\vspace{2.2\baselineskip}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 


==> settings/mytikzcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % mytikzcomments.tex
% %
% % 	requires:		\usepackage{tikz}
% % 				\usepackage{forloop}
% % 				\usepackage{arrayjobx}
% %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% compatibility
\pgfplotsset{compat=1.10}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% externalize tikz-figures as graphics
\usetikzlibrary{external}
\tikzexternalize[optimize command away=\includepdf] 
%externalize ignores \includepdf objects
% \tikzexternalize[mode=list and make,prefix=tmp/]
% \tikzset{external/mode=list and make}
\tikzsetexternalprefix{tmp/}
% \tikzexternaldisable

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% TikZ additional packages
% \usetikzlibrary{positioning,calc,intersections,arrows,3d,fit}
% \usetikzlibrary{shapes,snakes,spy}
\usetikzlibrary{shapes,spy,fit}
% \usepgfplotslibrary{patchplots}
% \usetikzlibrary{matrix,chains,scopes,fit,decorations.pathmorphing} % for sim chain
% \usetikzlibrary{shapes.geometric,shapes.arrows,decorations.pathmorphing}
% \usetikzlibrary{matrix,chains,scopes,positioning,arrows,fit}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PGF Plots additional packages
\usepgfplotslibrary{groupplots}
% \usepgfplotslibrary{fillbetween}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Font size in plots and graphics
\def\pgfplotfontsizetitle{\small}
\def\pgfplotfontsize{\footnotesize}
\def\tikzfontsize{\small}
\def\tikzfontsizesmall{\footnotesize}
\def\tikzfontsizetiny{\scriptsize}

\pgfplotsset{
  mystyle/.style ={%
    grid = major,
%     grid = none,
    every tick label/.append style={font=\pgfplotfontsize},
    every axis label/.append style={font=\pgfplotfontsize},
    legend style={font=\pgfplotfontsize},
    label style={font=\pgfplotfontsize},
    title style={font=\pgfplotfontsizetitle},
%       \pgfkeys{%
    /pgf/number format/set thousands separator = {}, % 1,000 -> 1000
%   }
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom drawing colors
% \definecolor{drawblue} {RGB}{87,117,225}
\colorlet{drawblue}      {blue!80!white}
% \definecolor{drawred}{RGB}{229,112,88}
\colorlet{drawred}       {red!80!white}
\colorlet{drawgray}      {gray}
% \definecolor{drawgreen}  {RGB}{0,.5,0}
\definecolor{drawgreen}  {RGB}{44,162,95}
% \definecolor{drawgreen}  {RGB}{49,163,84}
% \colorlet{drawgreen}  {olive}
\colorlet{drawpurple}    {purple}
\colorlet{draworange}    {orange}
\colorlet{drawlime}      {lime!80!black}
\colorlet{drawartichoke} {yellow!60!black}
\colorlet{TUGgray}{black!15}
\definecolor{TUGred}{RGB}{247,1,70}
\definecolor{IFBblue}{RGB}{51,112,169}
\definecolor{UTorange}{RGB}{191,87,0}
\definecolor{UTblue}{RGB}{0,95,134}
\definecolor{UTgreen}{RGB}{67,105,91}
\definecolor{UTgray}{RGB}{51,63,72}
\definecolor{UTyellow}{RGB}{242,169,0}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom basisfunction colors
\definecolor{basisColor1}{RGB}{59,76,192}
\definecolor{basisColor2}{RGB}{87,117,225}
\definecolor{basisColor3}{RGB}{119,154,247}
\definecolor{basisColor4}{RGB}{152,185,255}
\definecolor{basisColor5}{RGB}{184,208,249}
% \definecolor{basisColor6}{RGB}{213,219,230} % original settings
% \definecolor{basisColor7}{RGB}{236,211,197} % original settings
\definecolor{basisColor6}{RGB}{195,209,230}	% changed for printing
\definecolor{basisColor7}{RGB}{247,200,190}	% changed for printing
\definecolor{basisColor8}{RGB}{247,187,160}
\definecolor{basisColor9}{RGB}{244,154,123}
\definecolor{basisColor10}{RGB}{229,112,88}
\definecolor{basisColor11}{RGB}{203,62,56}
\definecolor{basisColor12}{RGB}{180,4,38}

\definecolor{basisColor8sw}{RGB} {189,189,189}
\definecolor{basisColor9sw}{RGB} {150,150,150}
\definecolor{basisColor10sw}{RGB}{115,115,115}
% \definecolor{basisColor11sw}{RGB}{82,82,82}
\definecolor{basisColor11sw}{RGB}{91,91,91}
\definecolor{basisColor12sw}{RGB}{37,37,37}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom plot colors and style

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initial set 0 (standard TikZ)
\colorlet{myblue}    {blue}
\colorlet{myred}     {red}
% \definecolor{mygreen} {RGB}{44,162,95}
\colorlet{mygreen}   {drawgreen}
\colorlet{mypurple}  {purple}
\colorlet{myorange}  {orange}


%%% Set 1 - dark colors
%%% http://colorbrewer2.org, number of data classes=3, middle color
%% \definecolor{myblue}  {RGB}{43,140,190}
% \definecolor{myblue}  {RGB}{43,140,190}
% \definecolor{myred}   {RGB}{227,74,51}
% \definecolor{mygreen} {RGB}{44,162,95}
% \definecolor{mypurple}{RGB}{197,27,138}
% \definecolor{myorange}{RGB}{217,95,14}

%%% Set 2 - light colors
%%% http://colorbrewer2.org, number of data classes=3, middle color
% \definecolor{myblue}  {RGB}{166,189,219}
% \definecolor{myred}   {RGB}{253,187,132}
% \definecolor{mygreen} {RGB}{153,216,201}
% \definecolor{mypurple} {RGB}{250,159,181}
% \definecolor{myorange}{RGB}{254,196,79 }


%%% Cycle lists for plots


%%% Cyclelist 1 (custom)
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   myblue,    every mark/.append style={solid, fill=.},mark=*          \\%
%   myred,     every mark/.append style={solid, fill=.},mark=square*     \\%
%   mygreen,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   mypurple,  every mark/.append style={solid, fill=.},mark=diamond*    \\%
%   % myorange,  every mark/.append style={solid, fill=.},mark=star    \\%
% }

% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   myblue,    dashed            \\%
%   myred,     dotted            \\%
%   mygreen,   dashdotted        \\%
%   mypurple,  dashdotdotted     \\%
%   myblue,    only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   myred,     only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   mygreen,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   mypurple,  only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%%% Cyclelist 2 (TikZ exotic)
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   teal,    every mark/.append style={solid, fill=.},mark=*           \\%
%   orange,  every mark/.append style={solid, fill=.},mark=square*     \\%
%   cyan,    every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   red,     every mark/.append style={solid, fill=.},mark=diamond*    \\%
%   % lime,  every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

% %%% Cyclelist 3 (TikZ standard)
% \pgfplotscreateplotcyclelist{mycyclelist}{
% %     \pgfplotscreateplotcyclelist{color}{%
% blue,every mark/.append style={fill=blue!80!black},mark=*\\%
% red,every mark/.append style={fill=red!80!black},mark=square*\\%
% brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
% black,mark=star\\%
% blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
% red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
% brown!60!black,densely dashed,every mark/.append style={
% solid,fill=brown!80!black},mark=square*\\%
% black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
% blue,densely dashed,mark=star,every mark/.append style=solid\\%
% red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
% % }
% %   blue,    every mark/.append style={solid, fill=.},mark=*           \\%
% %   red,     every mark/.append style={solid, fill=.},mark=square*     \\%
% %   brown,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   black,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%%% Cyclelist 4 (red styles)

% % \ifthenelse{\boolean{isbook}}{ 
% % % \definecolor{basisColor11new}{RGB}{203,80,56}
% % 
% % %% gray styles
% % \pgfplotscreateplotcyclelist{mycyclelist}{
% %   basisColor12sw,semithick, every mark/.append style={solid, fill=.},mark=*           \\%
% %   basisColor11sw,semithick, every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor10sw,semithick, every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor9sw , semithick,every mark/.append style={solid, fill=.},mark=diamond*    \\%
% %   basisColor8sw , semithick,every mark/.append style={solid, fill=.},mark=otimes    \\%
% % }
% % %% based on "linestyles*", pgfplots documentation S.199
% % % \pgfplotscreateplotcyclelist{mycyclelist}{
% % % semithick,darkgray,solid,        mark=*             \\%
% % % semithick,darkgray,dashed,       mark=square*       \\%
% % % semithick,darkgray,dotted,       mark=triangle*     \\%
% % % semithick,darkgray,dashdotted,   mark=diamond*      \\%
% % % semithick,darkgray,dashdotdotted,mark=otimes        \\%
% % % }
% % % %% copy of "black white", pgfplots documentation S.198 
% % % \pgfplotscreateplotcyclelist{mycyclelist}{
% % % every mark/.append style={fill=gray},mark=*\\%
% % % every mark/.append style={fill=gray},mark=square*\\%
% % % % every mark/.append style={fill=gray},mark=otimes*\\%
% % % mark=star\\%
% % % every mark/.append style={fill=gray},mark=diamond*\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=*\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=square*\\%
% % % % densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
% % % densely dashed,every mark/.append style={solid},mark=star\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=diamond*\\%
% % % }
% % % %% end copy
% % }{

%% red styles
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   basisColor12,semithick,   every mark/.append style={solid, fill=.},mark=*           \\%
%   basisColor11,semithick,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   basisColor10,semithick,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   basisColor9, semithick,   every mark/.append style={solid, fill=.},mark=+    \\%
%   basisColor8, semithick,   every mark/.append style={solid, fill=.},mark=otimes    \\%
% }
% % %
% % }

% %%% Cyclelist 5 comparison for trimmed cube example
\pgfplotscreateplotcyclelist{mycyclelist}{
blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,dashed,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
black,dashed,mark=star\\%
}


% \definecolor{cyclelistRed}{RGB}{228,26,28}
% \definecolor{cyclelistBlue}{RGB}{55,126,184}
% \definecolor{cyclelistGreen}{RGB}{77,175,74}
% \definecolor{cyclelistViolette}{RGB}{152,78,163}
% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   cyclelistRed,     semithick, solid               	\\%
%   cyclelistBlue,    semithick, loosely dashdotted        \\%
%   cyclelistGreen,   semithick, dashed      		\\%
%   cyclelistViolette,semithick, loosely dashdotdotted     \\%
%   cyclelistRed,     only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   cyclelistBlue,    only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   cyclelistGreen,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   cyclelistViolette,only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%% red and blue styles
% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   basisColor1,     semithick, solid               	\\%
%   basisColor10,    semithick, loosely dashdotted        \\%
%   basisColor3,   semithick, dashed      		\\%
%   basisColor12,semithick, loosely dashdotdotted     \\%
%   basisColor1,     only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   basisColor10,    only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   basisColor3,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   basisColor12,only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

% % \ifthenelse{\boolean{isbook}}{ 
% % %% gray styles
% % \pgfplotscreateplotcyclelist{mycyclelistcompare}{
% %   basisColor12sw, semithick, loosely dashdotdotted     \\%
% %   basisColor11sw, semithick, loosely dashed      		\\%
% %   basisColor10sw, semithick, dashed \\%loosely dashdotted        \\%
% %   basisColor9sw,  semithick, solid               	\\%
% %   basisColor12sw, only marks,   every mark/.append style={solid, fill=.},mark=otimes    \\%
% %   basisColor11sw, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor10sw, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor9sw,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
% % }
% % %
% % 
% % }{
%% red styles
\pgfplotscreateplotcyclelist{mycyclelistcompare}{
  basisColor12, semithick, loosely dashdotdotted     \\%
  basisColor11, semithick, loosely dashed      		\\%
  basisColor10, semithick, dashed \\%loosely dashdotted        \\%
  basisColor9,  semithick, solid               	\\%
  basisColor12, only marks,   every mark/.append style={solid, fill=.},mark=otimes    \\%
  basisColor11, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
  basisColor10, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
  basisColor9,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
}
% % %
% % }

% % \ifthenelse{\boolean{isbook}}{ 
% % %% gray styles
% % \tikzset{mycyclelistcompareReferenceA/.style={basisColor12sw,solid}}
% % \tikzset{mycyclelistcompareTestA/.style={basisColor12sw,only marks,mark=otimes}}
% % }{
%% red styles
\tikzset{mycyclelistcompareReferenceA/.style={basisColor12,solid}}
\tikzset{mycyclelistcompareTestA/.style={basisColor12,only marks,mark=otimes}}
% % }
% \pgfplotscreateplotcyclelist{mycyclelistcompareToReference}{
%   basisColor9, very thick, loosely dashed    \\%
%   basisColor12, solid\\%
% %   basisColor11, semithick, loosely dashed      		\\%
% %   basisColor10, semithick, dashed \\%loosely dashdotted        \\%
% %   basisColor9,  semithick, solid               	\\%
% %   basisColor12, only marks,mark=otimes    \\%
% %   basisColor11, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor10, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor9,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
% }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Additional styles

%% line styles
\tikzset{helpline/.style={thin,dashed}}
\tikzset{labelline/.style={thin}}
\tikzset{referencePath/.style={dotted,very thick}}
\tikzset{helparrow/.style={thin,arrows={-latex}}}
% \tikzset{pointer/.style={arrows={latex-latex}}}
\tikzset{pointer/.style={arrows={-latex}}}
\tikzset{axis/.style={thin,arrows={->}}}
\tikzset{force/.style={thick,arrows={->}}}
\tikzset{forceInverse/.style={thick,arrows={<-}}}
\tikzset{Gamma/.style={ultra thick}}
\tikzset{controlPoly/.style={draw=black}}
\tikzset{GammaFill/.style={fill=lightgray,fill opacity=0.3}}
\tikzset{colorDiri/.style={drawgreen}}
\tikzset{GammaFillDiri/.style={fill=drawgreen,fill opacity=0.5}}
\tikzset{initialgrid/.style={thin,gray}}
\tikzset{intersectioncurve/.style={dashed,thick}}
\tikzset{trimmingcurve/.style={thick}}
\tikzset{boundingbox/.style={dashed,}}
\tikzset{approx/.style={thick,line join=round,dashed}}
\tikzset{integrationRegionEdge/.style={dashed}}

%% point styles
\tikzstyle{anode}= [circle, inner sep=1.3pt, draw, fill=black]
\tikzstyle{gausspoint}=[shape=circle,draw=black,fill=black,inner sep=0.8pt]
\tikzstyle{controlPoint}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{abscissaPoint}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{anchorPoint}=[shape=circle,draw=black,fill=black,thin,inner sep=0pt,minimum size=1.5mm]
% \tikzstyle{anchorPointDeg}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{anchorPointDeg}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{trimmingIntersectionPoint}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{approxnode}= [circle, inner sep=1.5pt, draw, fill=black]
% \tikzstyle{characterNode}= [rectangle, inner sep=1.8pt, draw,thick,fill=white]
\tikzstyle{characterNode}= [shape=cross out,rotate=45, inner sep=1.8pt, draw,very thick,fill=white]

\tikzstyle{aPointPatchA}= [circle, inner sep=1.3pt, draw, fill=black]
\tikzstyle{aPointPatchB}= [circle, inner sep=1.3pt, draw, fill=white]
\tikzstyle{aPointModelSpace}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]


% \tikzstyle{anchorPoint}=[shape=circle,draw=black,fill=black,inner sep=0pt,minimum size=1.5mm]%, maximum size=1.5mm]
% \tikzstyle{anchorPointDisp}=[shape=circle,draw=black,fill=drawgreen,inner sep=0pt,minimum size=1.5mm]%, maximum size=1.5mm]
% \tikzstyle{collocPoint}=[shape=rectangle,draw=black,fill=black,thick,inner sep=0pt,minimum size=1.2mm] %, maximum size=1.2mm] 
% \tikzset{Diri/.style={drawgreen}}
% \tikzset{Neum/.style={drawpurple}}
% \tikzset{collocNeum/.style={collocPoint, fill=drawgreen}}
% \tikzset{collocDiri/.style={collocPoint, fill=drawpurple}}
% 
% \tikzset{GammaDiri/.style={Gamma, Diri}}
% \tikzset{GammaNeum/.style={Gamma, Neum}}
% 
% \tikzset{anchorNeum/.style={anchorPoint, fill=drawpurple}}
% \tikzset{anchorDiri/.style={anchorPoint, fill=drawgreen}}
% 
% \tikzset{helpline/.style={thin,dashed}}
% \tikzset{helpline/.style={thin}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% help makro for convergence plots

\def\trianglecolor{black}
\newcommand{\upperSlopeTriangle}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \upperSlopeTriangle{2}{100}{1000}{5000}
{
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^#1) } node (A1) [pos=1] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{   #2  / (#3^#1)} node (A2) [pos=1] {} node [anchor=south,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=west,pos=0.5,black] {\tikzfontsizetiny #1};
}

\newcommand{\lowerSlopeTriangle}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \lowerSlopeTriangle{2}{100}{1000}{5000}
{
% 	\def\trianglecolor{black}
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^#1) } node (A1) [pos=0] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{   #2  / (#4^#1)} node (A2) [pos=0] {} node [anchor=north,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=east,pos=0.5,black] {\tikzfontsizetiny #1};
}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% B-spline functions

\newcounter{itR}
\newcommand{\bsplinevalue}[5] % input: #1 knot vector #2 order,  #3 intrinsic coordinate #4 span index #5 output name
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinevalue{\vKnots}{×}{×}{×}{×} fails!  )
{                    				
	\newarray\vKnots
	\newarray\vN
	\newarray\vNumeratorL
	\newarray\vNumeratorR
	\newarray\vSave

	\readarray{vKnots}{#1}
	\readarray{vN}{1}
	\readarray{vSave}{0}
	\readarray{vNumeratorL}{0}
	\readarray{vNumeratorR}{0}

	\foreach \j in {1,...,#2}
	{        
		\pgfmathparse{ int(#4+\j+1) } \checkvKnots(\pgfmathresult)
		\pgfmathsetmacro{\numR}{\cachedata-#3}
		
		\pgfmathparse{ int(#4-\j+2) } \checkvKnots(\pgfmathresult)
		\pgfmathsetmacro{\numL}{#3-\cachedata} 					

		\expandarrayelementtrue
		\pgfmathparse{ int(\j+1) }
		\vNumeratorL(\pgfmathresult)={\numL}
		\vNumeratorR(\pgfmathresult)={\numR}
		
		\forloop[1]{itR}{0}{\value{itR} < \j }
		{
			\pgfmathparse{ int(\theitR+1) } \let\tS\pgfmathresult  	
			\checkvSave(\tS)							
			\pgfmathsetmacro{\save}{\cachedata}  
		
			\pgfmathparse{int(\j-\theitR+1)} \checkvNumeratorL(\pgfmathresult)
			\pgfmathsetmacro{\tmpL}{\cachedata} 	
		    
			\pgfmathparse{ int(\theitR+2) } \checkvNumeratorR(\pgfmathresult)
			\pgfmathsetmacro{\tmpR}{\cachedata} 	       
	
			\pgfmathparse{ int(\theitR+1) } \checkvN(\pgfmathresult)
			\pgfmathparse{ \cachedata / (\tmpL+\tmpR) } \let\tmp\pgfmathresult
			
			\pgfmathparse{ \save + \tmpR * \tmp } 
			\vN(\tS)={\pgfmathresult}

			\pgfmathparse{ \tmpL * \tmp } \let\tmpsave\pgfmathresult
			\pgfmathparse{ int(\theitR+2) } \let\tS\pgfmathresult      
			\vSave(\tS)={\tmpsave}
		}
		
		\pgfmathparse{ int(\j+1) } \checkvSave(\pgfmathresult )
		\vN(\tS)={\cachedata}
	}

	% write to return argument #5
	\pgfmathparse{int( #2+1) } \let\lastIndex\pgfmathresult
	\checkvN(1) \pgfmathsetmacro{\first}{\cachedata}  
	\foreach \i [remember=\a as \lasta (initially \first)] in {2,...,\lastIndex}
	{
		\checkvN(\i) \def\a{\lasta,\cachedata} 
		% store \a of last loop
		\ifthenelse{\i=\lastIndex}{ \xdef#5{\a} }{}
	}
    
	% clean up
	\foreach \i in {1,...,\lastIndex}
	{
	    \clrarray{vNumeratorR}(\i)
	    \clrarray{vNumeratorL}(\i)
	    \clrarray{vN}(\i)
	    \clrarray{vSave}(\i)
	}
	\delarray\vN
	\delarray\vNumeratorL
	\delarray\vNumeratorR
	\delarray\vSave
}

\newcounter{countvalues}
\newcounter{getBasis}
\newcommand{\bsplinebasis}[4] % input: #1 knot vector, #2 order,  #3 id of basis function, #4 output
{						% example: \bsplinebasis{0&0&0&1&2&2&2}{2}{0}{\output}
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinebasis{\vKnots}{×}{×}{×} fails!  )
						%		countvalues returns the number of non-zero basis functions
						%		\output ''intrinsic Coord, basis function value'': ''u0,N_#3(u0)'',''u1,N_#3(u1)'',...,''un,N_#3(un)''
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}

    \pgfmathparse{#3}  \let\i\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult

    % loop over support of N_i
    \setcounter{countvalues}{0}
    \setcounter{getBasis}{\p} %\addtocounter{getBasis}{1}
    \pgfmathparse{int(\i+\p)}
    \foreach \knotspan in {\i,...,\pgfmathresult}
    {
        % check span size
	\pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
	\pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
	
	\pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
	\pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL

	\pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
   
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
		\pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult

		% get all non vanishing basis functions
		\bsplinevalue{#1}{\p}{\u}{\knotspan}{\Basis} 
		\def\basisfuncarray{{\Basis}} 				% remark index start from 0
		
		\pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
		
		\ifthenelse{\thecountvalues=0}
		{ 
			\xdef\nodeB{"\u,\pgfmathresult"}
		}{
			\xdef\nodeB{\nodeB,"\u,\pgfmathresult"}  
		}
		\addtocounter{countvalues}{1}
            }
        }{}
        \addtocounter{getBasis}{-1}
    }
    
	\xdef#4{\nodeB}

	\delarray\vKnots
}


\newcommand{\bsplinebasisspan}[6] % input: 	#1 knot vector, #2 order,  #3 segment id of basis function within (#4), 
{							% 		#4 id of knot span,  #5 id of plotted span, #6 output
							% example: \bsplinebasis{0&0&0&1&2&2&2}{2}{0}{\output}
							% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinebasis{\vKnots}{×}{×}{×} fails!  )
							%		#3 is not  the basis function id 
							%		   - for each span the numbering start at 0 - index first non-zero basis function of #4
							%		countvaluesspan returns the number of non-zero basis functions
							%		\output ''intrinsic Coord, basis function value'': ''u0,N_#3(u0)'',''u1,N_#3(u1)'',...,''un,N_#3(un)''
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}

    \pgfmathparse{#5}  \let\plotknotspan\pgfmathresult
    \pgfmathparse{#4}  \let\splineknotspan\pgfmathresult
    \pgfmathparse{#3}  \let\i\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult

    % only one iteration over support '\plotknotspan' 
    % evaluation the polynome defined over '\splineknotspan'
    \setcounter{countvalues}{0}
    \setcounter{getBasis}{\i} 
    \foreach \knotspan in {\plotknotspan}
    {
        % check span size
	\pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
	\pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
	
	\pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
	\pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL

	\pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
   
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
		\pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult

		% get all non vanishing basis functions
		\bsplinevalue{#1}{\p}{\u}{\splineknotspan}{\Basis} 
		\def\basisfuncarray{{\Basis}} 				% remark index start from 0
		
		\pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
		
		\ifthenelse{\thecountvalues=0}
		{ 
			\xdef\nodeB{"\u,\pgfmathresult"}
		}{
			\xdef\nodeB{\nodeB,"\u,\pgfmathresult"}  
		}
		\addtocounter{countvalues}{1}
            }
        }{}
        \addtocounter{getBasis}{-1}
    }
    
	\xdef#6{\nodeB}

	\delarray\vKnots
}





\newcommand{\plotbsplinebasis}[4] 	% input: #1 knot vector, #2 order,  #3 id of basis function, #4 plot settings
{							% example: \plotbsplinebasis{0&0&0&1&2&2&2}{2}{0}{green,smooth}
							% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  )
	% calculate B-spline values
	\bsplinebasis{#1}{#2}{#3}{\nodeOut}
	\def\nodearray{{\nodeOut}}

	% store B-spline values into coordinates and save their name
	\xdef\name{ }
	\addtocounter{countvalues}{-1}
	\foreach \i in {0,...,\thecountvalues}
	{
		\pgfmathparse{\nodearray[\i]}
		\coordinate (point\i) at (\pgfmathresult);	  
		\xdef\name{ \name (point\i)  }
	}
	
	% plot basis
	\draw[#4] plot coordinates{ \name };
	
	% reset coordinates
	\xdef\name{ }
}


\newcommand{\plotbsplinesegment}[6] 	% input: 	#1 knot vector, #2 order,  #3 segment id of basis function within (#4),  
{								%		#4 id of knot span, #5 id of plotted span, #6 plot settings
								% example: 
								%	->normal B-spline plot
								% 	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{1}{basisColor3,dotted,thick}
								%	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{2}{basisColor5,dotted,thick}
								%	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{3}{basisColor7,dotted,thick}
								%	
								%	-> plot the B-spline segments 0,1,2 of span 3 in span 2
								%
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{0}{3}{2}{red,smooth}
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{1}{3}{2}{red,smooth}
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{2}{3}{2}{blue,smooth}
								%
								% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  
								
	% calculate B-spline values
	\bsplinebasisspan{#1}{#2}{#3}{#4}{#5}{\nodeOut}
	\def\nodearray{{\nodeOut}}

	% store B-spline values into coordinates and save their name
	\xdef\name{ }
	\addtocounter{countvalues}{-1}
	\foreach \i in {0,...,\thecountvalues}
	{
		\pgfmathparse{\nodearray[\i]}
		\coordinate (point\i) at (\pgfmathresult);	  
		\xdef\name{ \name (point\i)  }
	}
	
	% plot basis
	\draw[#6] plot coordinates{ \name };
	
	% reset coordinates
	\xdef\name{ }
}


\newcommand{\plotbsplineaccumulated}[5] 	% input: 	#1 knot vector, #2 order,  #3 subdivision coefficient,  
{						%		#4 id of knot span,  #5 plot settings
						% example: 
                                                %       ->plot non-zero basis function segment within #4
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{1&0&0}{3}{red,smooth}
						% 	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&1&0}{3}{green,smooth}
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&0&1}{3}{blue,smooth}
                                                %       
                                                %       ->plot weighted combination of basis function segments within #4
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&1&1}{3}{blue,smooth}
						%	
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                                            
    %% calculate B-spline values and compute their weighted sum using vSubCoef
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}
    \newarray\vSubCoef 	% remark index start from 1
    \readarray{vSubCoef}{#3}
    
    \pgfmathparse{#4}  \let\plotknotspan\pgfmathresult
    \pgfmathparse{#4}  \let\splineknotspan\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult
    
    % only one iteration over support '\plotknotspan' 
    % evaluation the polynome defined over '\splineknotspan'
    \setcounter{countvalues}{0}
    \pgfmathparse{int( \p+1) } \let\lastIndex\pgfmathresult
    \foreach \knotspan in {\plotknotspan}
    {
        % check span size
        \pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
        \pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
        
        \pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
        \pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL
        
        \pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
        
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
                \pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult
                
                % get all non vanishing basis functions
                \bsplinevalue{#1}{\p}{\u}{\splineknotspan}{\Basis} 
                \def\basisfuncarray{{\Basis}} 				% remark index start from 0
                
                \setcounter{getBasis}{0} 
                \pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
                \let\basisValue\pgfmathresult
                
                \checkvSubCoef(1) \pgfmathsetmacro{\coef}{\cachedata}  
                \pgfmathparse{ \basisValue * \coef } \let\first\pgfmathresult
                
                \xdef\lastx{\first}
                \foreach \i in {2,...,\lastIndex}
                { 
                    \addtocounter{getBasis}{1}       
                    \pgfmathparse{\basisfuncarray[\thegetBasis]}
                    \let\basisValue\pgfmathresult
                    
                    \checkvSubCoef(\i) \pgfmathsetmacro{\coef}{\cachedata}  
                    \pgfmathparse{ \lastx + \basisValue * \coef } \let\sum\pgfmathresult
                    
                    \xdef\lastx{\sum}
                    
                    % store \a of last loop
                    \ifthenelse{\i=\lastIndex}
                    {
                        \ifthenelse{\thecountvalues=0}
                        { 
                            \xdef\nodeBB{"\u,\sum"}
                        }{
                            \xdef\nodeBB{\nodeBB,"\u,\sum"}  
                        }
                        \addtocounter{countvalues}{1}
                    }{}
                    
                }
            }
        }{}
    }
    
    \delarray\vKnots
    \delarray\vSubCoef
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    %% plot accumulated values
    \def\nodearray{{\nodeBB}}
    
    % store B-spline values into coordinates and save their name
    \xdef\name{ }
    \addtocounter{countvalues}{-1}
    \foreach \i in {0,...,\thecountvalues}
    {
        \pgfmathparse{\nodearray[\i]}
        \coordinate (point\i) at (\pgfmathresult);                
        \xdef\name{ \name (point\i)  }
    }
    
    % plot basis
    \draw[#5] plot coordinates{ \name };
    
    % reset coordinates
    \xdef\name{ }
}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 


==> settings/settings_font.tex <==
\usepackage[utf8]{inputenc} % for UTF-8 encoding
\usepackage[german,english]{babel}  
\usepackage[T1]{fontenc} % größerer Zeichenvorat z.B. für Umlaute 
\usepackage{lmodern} % latin modern fonts - added to resolve visualization issues with fontenc

% \usepackage{times} % times font
% \usepackage{mathptmx}  % times roman, including math (where possible)

%%% Hyphenations 
%\hyphenation{fast-bem}
% 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> settings/settings_math.tex <==
\usepackage[intlimits]{amsmath}
\usepackage{amssymb} 
\usepackage{amsthm}
% \usepackage{amsbsy}
\usepackage{amsfonts,mathrsfs}
\usepackage{bm}
% \usepackage{mathdots} % for \iddots
\usepackage{mathtools} % for \coloneqq and \shortintertext


%%%% Tensors, Matrices and Vectors
% \usepackage[arrow]{hhtensor}
% \usepackage[uline]{hhtensor}
% \usepackage[bold]{hhtensor}
%%%%%%%%%%%

\usepackage{siunitx} %% units

% \usepackage{amsfonts,mathrsfs,bbm}
% \usepackage{amsfonts,mathrsfs}

%\usepackage{mathrsfs} 
%\usepackage{nicefrac}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "fastigabem"
%%% eval:
%%% End: 


==> settings/settings_tools.tex <==
%%% TikZ Stuff
\usepackage{tikz}
\usepackage{tikz-3dplot}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{tikzscale}
\usepackage{standalone} % for standalone compilation of tikz graphics

%%% TikZ B-spline plots
\usepackage{forloop}
\usepackage{arrayjobx}

%%% algorithms
\usepackage[noend]{algorithmic}
\usepackage{algorithm}

\usepackage{booktabs} % for tables: toprule, midrule, bottomrule
\usepackage{hyperref} % for links -> this will be loaded by pdfcomment package
% \usepackage{calc}
\usepackage{xspace} % horizontal space after makro words

%% packages for authors' notes
\usepackage{xcolor,pdfcomment,soul} % add pdf comments
\usepackage[textsize=footnotesize]{todonotes}
% \usepackage[textsize=footnotesize,textwidth=1.2cm]{todonotes}
% \setlength{\marginparwidth}{1.2cm}

%%% subcaptions for figures
\usepackage{subcaption} 			%% 1a
\usepackage[labelformat=simple]{subcaption}   	%% 1(a)
\renewcommand\thesubfigure{(\alph{subfigure})}	%% 1(a)

\usepackage{enumerate} %% symbols for enumeration


% \usepackage{listings} %% enviroment for code formating 
